Exploiting Pointer Analysis in Memory Models for Deductive Verification

Cooperation between verification methods is crucial to tackle the challenging problem of software verification. The paper focuses on the verification of C programs using pointers and it formalizes a cooperation between static analyzers doing pointer analysis and a deductive verification tool based on first order logic. We propose a framework based on memory models that captures the partitioning of memory inferred by pointer analyses, and complies with the memory models used to generate verification conditions. The framework guided us to propose a pointer analysis that accommodates to various low-level operations on pointers while providing precise information about memory partitioning to the deductive verification. We implemented this cooperation inside the Frama-C platform and we show its effectiveness in reducing the task of deductive verification on a complex case study.

==> mm-env.tex <==
%!TEX root = main.tex

\section{Memory Model Environment}
\label{sec:mme}
The abstract memory model $\ammem$ used in this semantics
is represented by a \emph{memory model environment} (called simply environment)
that keeps the information required by the VC generation, for example the current
set of variables used for modeling the state at the current point.
%
Figure~\ref{fig:lmm} defines a \emph{signature for memory model environments}
that captures the essential features required by the
compilation of statements in our toy language into VC formulas.
In the next sections, we supply several memory model environments
that demonstrate the abstraction capabilities of this signature.


\begin{figure}[ht]
$\begin{array}{lrll}
\mbox{Types}
& \mmmem, & \mmloc %%\\ \triangleq & \mmblk \times \mathcal{E},
 \\
& \mmval \triangleq & \mmvint(\lterms_\lintegers) \mid \mmvptr(\mmloc) %\mid \mathtt{Vundef} 
\\[2mm]
\mbox{Constants} 
& \mmemp : & 2^\cvars \ft \mmmem 
\\[2mm]
\mbox{Operations} 
& \mmbase : & \cvars \ft \mmloc 
\\
& \mmshft : & \mmloc \ft \lterms_\lintegers \ft \mmloc_\bot 
\\[1mm]
%% MS: this is a programming interface and the functions shall be partial
%%     the undefined cases have been dealt using alarms
%%     but some environments may not provide them
%& \mmalloc : & \mmmem \ft \mathcal{E} \ft \mmmem \times \mmloc \\
%& \mmfree  : & \mmmem \ft \mmloc \ft \mmmem \\
& \mmload  : & \mmmem \ft \cscalar \ft \mmloc \ft \mmval_\bot \\
& \mmstore : & \multicolumn{2}{l}{\mmmem \ft \cscalar \ft \mmloc \ft \mmval \ft
               (\mmmem \times \lterms_\lbools)_\bot} \\
\end{array}$
\caption{Interface for memory model environments}
\label{fig:lmm}
\vspace{-2eX}
\end{figure}


The signature in Figure~\ref{fig:lmm} should be compared with
the abstract memory model from Figure~\ref{fig:am}.
%
The environment shall define
a type $\mmmem$ providing information about the state of the memory and
a type $\mmloc$ encoding information on memory locations.
%By omitting memory blocks from this signature,
%we permit a more abstract relation between memory locations and
%program variables, based only on the operation $\mmbase$.
This abstraction allows to define an efficient environment for
programs with or without pointer manipulation.
%
The environment shall provide a type for basic values
stored in the memory: integers and locations. The integer values are
specified by integer terms in $\ltheory$, denoted by $\lterms_\lintegers$.
%
The empty environment for a set \texttt{V} of active program variables
is provided by $\mmemp(\texttt{V})$.

%
The arithmetic operation on locations is encoded in
operation $\mmshft$, if this operation is supported by
the memory model. Indeed, we use an error monad with error value $\bot$
for the result type of some operations to point out
that these operations may be defined only under some conditions
%by an environment 
(\eg, no dereference, no alias, variable used only by reference, ...).
We provide in Section~\ref{ssec:simple} an example
of environment where the operation $\mmshft$ is undefined.
%
The updating of the memory environment $\mmstore$ produces a
new environment and a formula in $\ltheory$, in the set $\lterms_\lbools$.%
\footnote{In languages with conditionals, environments should also provide a function $\mmjoin : \mmmem \ft
\mmmem \ft \mmmem \times \lterms_\lbools$ which is used to join execution paths.
It returns the new environment to use and a set of equalities
which make the environments equal. % \textcolor{red}{%
% We omit this feature from the signature because our toy language does not
% include decision statements.}
}


==> notes.tex <==
All pair (input,output) are disjoint pairwise.
All pair (output,output) are disjoint pairwise.


==> overview.tex <==
\section{Overview}

In this section, we present in an informal way our analysis.

\subsection{Typed Memory Model}

\begin{figure}
\begin{lstlisting}[language=C]
typedef struct { uint8_t sig; float val } data_t;
typedef struct { uint8_t src; uint8_t dst } perm_t;
struct {
  data_t *in1, *in2, *in3, ...;
  data_t *out1, *out2, *out3, ...;
  perm_t *perm1, *perm2, *perm3, ...;
};

\end{lstlisting}

\caption{Interesting example}
\end{figure}

The memory model used in the \textsf{WP} plug-in is a type-indexed
memory model restricted to the well-typed subset of a programming
language. The separation of memory regions is done according to the
set of types $\cstyp$ of memory locations, which is similar to ``component
as array'' model of Burstall-Bornat. Moreover, this model assumes
that all fields of a structure are implicitely separated since pointer
casting and unions are not allowed in the source language. A location
is represented in the standard way as a pair of a base and offset,
$(b_{\cvar},o)$,where $b_{\cvar}$models the base of program variable
$\cvar$ and $o$ an offset. Therefore, the memory is a bounded collection
of typed arrays from locations to locations or scalar values (given
the access type). Using the array theory, this model is highly scalable
but provers are unable to prove satisfiability for programs where
aliasing occurs within the same type.

\subsection{Separation by Static Analysis}

\subsubsection{Base separation}

The \textsf{EVA} implements a static value analysis based on the principles
of abstract interpretation. Abstract interpretation links a \emph{concrete}
semantics, typically the set of all possible executions of a program,
to a more coarse-grained, \emph{abstract} semantics. Any program transformation
must have an abstract encoding that captures all possible outcomes
defined by the concrete semantics. This ensures that the abstract
semantics is a sound approximation of the runtime behavior of the
program. For each instruction of the program, \textsf{EVA} computes
an over-approximation of all memory locations involved in that instruction.
We use the over-approximation inferred for state and pointer values
as a \emph{points-to} information.

Pointers are seen as offsets with respect to a symbolic block location
called \emph{b}ase and have no relation with the locations in the
virtual memory space used during the concrete execution. Blocks of
different bases are implicitly separated: it is impossible to move
from the block of one base to another using pointer arithmetic. We
build a memory model using the bounded set of symbolic blocks as regions
and points-to information to dispatch those locations amongst the
possible regions. Those regions offer a finer grain of separation
than the typed one but not sufficient enough in case of compound types.

\subsubsection{Alias Analysis}

We implemented an alias analysis on top of the \textsf{EVA} value
analysis. The latter infer at each program point $\cstmt$, for all
left-values $\clval$ in $s$ an over-approximation of the slices
of memory that $lv$ could belong in the form of a \emph{zone,} i.e.,
a mapping to symbolic bases to slices in the block corresponding to
those bases (using an abstraction for offsets). Given those zones,
we can infer better separation by providing an equivalence relation
between left-values such that the zone of any left-value should belong
to one and only one equivalence class. This analysis cannot degenerate
since the maximal equivalence class is the union of zones of all left-values.

We refine our model by doing a product between the base separation
above and the alias analysis, using again state and value abstraction
as points-to information.

\subsubsection{Cells Analysis}

We experimented a naive analysis given a separation by aggregates.
Recall that zones' bindings are symbolic bases, we collect the bindings
for all left-values syntactically present in the function. Structures
are flatten as aggregates.

\subsection{A functor model for Region Analysis}

We propose a new memory model parametrized by a static analysis whose
separations and points-to relations are inferred by the analysis.
We suppose that we are given a value abstraction able to give an over-approximation
of all possible values of expressions and concrete locations pointed
by an address in a given state, as well as abstract semantics of the
operations on those values (pointer arithmetic, shifting, ...). The
static analysis also provides a state abstraction holding for each
program point the set of possible concrete states, along with the
abstract semantic for the dereference of l-values. The abstracts semantics
should be a sound approximation of the runtime behavior of the program.


==> pointer-abstract.tex <==
%!TEX root = main.tex

\section{Comparing Pointer Analyses}

Abstract interpretation for C programs usually represent pointers
as an abstraction for the bases that may be pointed, plus a numerical
abstraction for the offset (expressed in bytes). More ``symbolic''
abstractions for the offset are uncommon, due to the possibility of
performing pointer arithmetics (thus breaking any semblance of structure
in the offset). Depending on the coarseness of the abstract chosen
for the offset, spurious values may be obtained -- values that do
not correspond to possible values in the concrete. The numerical abstraction
often uses congruences (directly of through a reduced product) to
represent pointers to arrays precisely, but this is usually insufficient
for pointers ranging to possibly multiple fields of a structure. In
the following example, if $p$ can range over $s.m$, $s.n$ and $s.p$,
a congruence abstraction will lead to the additional (spurious) value
$s.o$ where \code{struct \{ int m, n, o, p, q\} s;} 

We call \emph{exact} an abstract operator that introduces no additional
loss of precision compared to the concrete operation. Formally given
$f$ and $f^{\sharp}$ its equivalent in the abstract, $f^{\sharp}$
is exact if $\forall x^{\sharp},\gamma(f^{\sharp}(x^{\sharp}))=\left\{ f(x),x\in\gamma(x^{\sharp})\right\} $.
It is important to understand which operations involving pointers
are exact (and which are not). Imprecisions in this part of the analysis
translates directly to a coarser memory model in the deductive verification
side -- leading to more complex proof obligations. We are going to
illustrate this on the computation of \code{(IN[i])->s}, 
where $i\in\left\{ 0..8\right\} $,
\code{typeof(IN)=AS_t**}, and \code{typedef struct{float v; char s;} AS_t;} 
\begin{enumerate}
\item The computation of \code{&IN[i]} is done as \code{((char*)IN)+i*sizeof(AS_t*)}.
	Since \code{sizeof(AS_t*)} is a constant, this operation can be done exactly
	when offsets are represented using congruences. 
\item Computing \code{IN[i]} involves querying the memory abstraction for the
	base \code{IN}, at all the offsets returned in the previous computation.
	The result is the join of the pointer abstractions contained at each
	location. Depending on the contents of \code{IN}, multiples bases can be
	returned, each possibly with multiple offsets. In particular, the
	joins of the possible offsets are often re-abstracted. This operation
	is thus \emph{not} exact. Furthermore, the analyser may chose to abstract
	even more (i.e. go to $\top$) when $i$ ranges over too many possible
	values.
\item The computation of \code{&(IN[i]->s)} consists in shifting the abstraction
found at the previous step by sizeof(float) bytes. This operation
is exact if offsets are represented using congruences.
\item The (final) computation \code{(IN[i]->s)} involves querying the memory abstraction
at the bases and offsets found in step 3. As in step 2, this operation
is in general not exact, because the joing operator is used to merge
the abstractions found at each pair base $\times$ offset.
\end{enumerate}
When translating pointers to DV, we only use phases 1 to 3. Hence,
only phase 2 can introduce spurious abstractions. In Frama-C/Eva,
two additional properties mitigate this loss of precision. First,
the analyzer never goes to $\top$ when the abstraction for $i$ is
too large. Second, pointers are not abstracted as a pair of abstract
bases and abstract offsets $(B^{\sharp},o^{\sharp})$, but as a set
of possibles bases, together with an abstract offset for \emph{each}
base: $\left\{ b_{1}+o_{1}^{\sharp},\,b_{2}+o_{2}^{\sharp},\,\dots\right\} $.
As a consequence, the operation is not exact only when the join operator
on abstract offsets introduces spurious concretizations. Frama-C/Eva
offers the possibility to remove this last source of inaccuracy,
by using \emph{small sets of integers} instead of congruences. Small
sets of integers are exact until the abstractions reaches a cardinality
of $k$, in which case they automatically degenerate into congruences.
This limit $k$ is user-settable, through option \code{-val-ilevel}. We
take advantage of this possibility in our experiments, and consider
proof obligations obtained (1) when all pointers abstractions are
exact; (2) when some spurious pointer values are introduced.


==> proposal.tex <==
\section{Proposals}
\subsection{MME Shift 1st proposal}
\[\mathbf{sig}~\mathsf{PA}\,: \\
\quad
\begin{array}[t]{rl}
    \mathbf{type}~ 
    & \mmvdloc \\
    \mathbf{ops}~ 
    & \mmvdfont{base} : \cvars \to \mmvdloc \\
    & \mmvdfont{shift} : \mmvdloc \to \lterms_\lintegers \to \mmvdloc \\
    & \mmvdfont{domain} : \mmvdloc \ft \pset{\mmvdblk} \\
    & \mmvdfont{extract} : \mmvdloc \ft \mmvdblk \ft \mmvdloc
\end{array}\quad
\begin{array}[t]{rl}
    \mathbf{type}~
    & \mmvdst \\
    \mathbf{ops}~
    & \mmvdfont{load} : \mmvdst \to \cptrtyps \to \mmvdloc \to \mmvdloc
\end{array}\quad
\begin{array}[t]{rl}
    \mathbf{type}~
    & \mmvdblk \\
    \mathbf{ops}~ 
    & \mmvdfont{base} : \mmvdblk \ft \cvars
    \\
    & \mmvdfont{slice} : \mmvdblk \to \lterms_\lintegers \to \lterms_\lbools
\end{array}
\]


\[
    \{ \absloc_i \mid \exists \mathabs{b}_i, \absloc_i =
    \mmvdfont{extract}(\mathabs{b}_i, \absloc)
\wedge \mathabs{b}_i \in \mathsf{PA}.\mmvdfont{domain}(\absloc) \}
\]

\[
    \{ \absloc_{i_s} = \mathsf{PA}.\mmvdfont{shift}(\absloc_i, e_o) \}
\]

Shifting on a unique symbolic base:
\[
\mathsf{PA}.\mmvdfont{domain} (\absloc_{i_s})=\{\mathabs{b}_{i_1},\ldots,\mathabs{b}_{i_n}\}
\]

\[
e'_{b_i} \ \triangleq\ \left(\begin{array}{ll}
        \mathsf{PA}.\mmvdfont{slice}(\mathabs{b}_{i_1},\logic{e_o+e})
        \logic{~?~\mathabs{b}_{i_1} ~:~} \\ \quad{\ddots}\  %\\\quad\quad
        \mathsf{PA}.\mmvdfont{slice}(\mathabs{b}_{i_{n-1}},\logic{e_o+e})\logic{~?~\mathabs{b}_{i_{n-1}}~:~
        \mathabs{b}_{i_n}}
\end{array}\right)
\]


\[
\mathsf{PA}.\mmvdfont{domain} (\absloc_{s})=\{\mathabs{b}_{1},\ldots,\mathabs{b}_{n}\}
\]

\[
e'_{b} \ \triangleq\ \left(\begin{array}{ll}
        e_b = \mathabs{b}_1\logic{~?~e'_{b_1} ~:~} \\ \quad{\ddots}
        e_b = \mathabs{b}_{n-1}\logic{~?~e'_{b_{n-1}} ~:~}b_n
\end{array}\right)
\]

\paragraph{BO}
\[
\mmvdfont{extract}(\absloc, \mathabs{b})\triangleq
\{(\mathabs{b_v}, \mathabs{i})\mid \mathabs{b_v} = \mathabs{b}\}
\]

\paragraph{C}

